Combining Neuro-Evolution of Augmenting Topologies with Convolutional Neural Networks

Current deep convolutional networks are fixed in their topology. We explore the possibilites of making the convolutional topology a parameter itself by combining NeuroEvolution of Augmenting Topologies (NEAT) with Convolutional Neural Networks (CNNs) and propose such a system using blocks of Residual Networks (ResNets). We then explain how our suggested system can only be built once additional optimizations have been made, as genetic algorithms are way more demanding than training per backpropagation. On the way there we explain most of those buzzwords and offer a gentle and brief introduction to the most important modern areas of machine learning

==> sections/contact_with_doctors.tex <==
Not much time has passed after the planning until we already began looking for doctors who could cooperate with us on the project. \\
For this purpose we sought doctors who were active exclusively in the field of oncology. \\
The term oncology is reffered to the branch of medicine that deals with the diagnosis, treatment and prevention of different types of cancer (tumor disease). \\
With our project being almost entirely about breast mammography, we needed doctors which are specialized in the field of oncology, more specific - breast oncology.  
According to this categorization we then proceeded.\\
After some research on the internet and also in books, we finally cut down 26 doctors who could be considered qualified to for the project. \\
We have sent all of the doctors a brief description of our project. We explained to them the core and the content of the project. Some of them answered the e-mails we sent.  \\
Most of the doctors have too much research to do, thus they just don't have as much time. \\
We arranged a few appointments, which were unfortunately not in the time span of our project. \\
Two doctors sent us a study protocol request, which means they required a protocol of our project that is extremely detailed. \\
We wrote the following protocol and sendt it to the doctors. \\
This we sent the doctors. \\
Dr. Serafino Forte of the hospital of Baden has invited us to the hospital after examining the study protocol. \\
We talked to him about all the details in medical and organizational terms. At first he looked at our mammography record. Immediately he realized that our mammographys are obsolete, because this technology is no longer needed and probably outdated. \\
Our data was in the old format of the film-film system. This was good for our project on the one hand but on the other hand it didn't speak so good. \\
It is definitely an advantage, because we have the possibility to have different mammographys evaluated. \\
However, it has a disadvantage too. \\
It is very difficult to get to the new mammographys because we need a lot of mammographys to train our software, we have to submit an ethics application. \\
This is an even more detailed application than the study protocol, which is checking if our project is as trustworthy as possible. \\
The application is examined by the Swiss Ethics Committees for Human Research. \\
In this application the financial resources are examined. \\
The financial resources are checked because the application is not free of charge. \\
To submit an application, you have to pay a basic flat rate of 800.00 CHF. \\
A check should be made for how well can the people be put together.
This means that four individuals working as a team could possibly carry out such a project because at the end of it it's just a product, resulting from months of work. \\
Apart from the organizational, we have also looked at the medical aspects as mentioned earlier in the chapter. \\
For Dr. Serafino Forte, it was quite important that our software could not only tell you whether a person is diagnosed with cancer, but also what type of cancer does he have. \\


==> sections/convolutional_neural_networks/problems_with_image_recognition.tex <==
Most neural networks are unable to handle the amount of data contained in an image.
For example an image with a resolution of 3264x2448 (8 Megapixels) would result in almost 24 million inputs, as each pixel is split into its red, green and blue parts.

Another challenge is the detection of so called "features" across an image. Traditional neural networks only detect a feature at a specific location in the image.
This is a big issue in image recognition, as you almost always want the entire image to be handled equally.
A self-driving car should recognize a stop sign, regardless of its position in the image.


==> sections/initial_position.tex <==
- The project took off with a semi-finished NEAT-library\\
- There is a library named "Hippocrates" consisting of approximately a half a year of work



==> sections/integration_tests.tex <==
We use automated testing to check each code change for issues. This means that the code everyone works on is located in a separate git branch \cite{gitbranch} and has to pass all integration tests before it gets merged into the main branch. A branch can be seen as a copy of the project that one works on in parallel to the original. When the work is done, the changes are copied over to the original version.

But before the changes can be added to the main branch, they have to pass our tests, which are basically dummy-programs that get executed on Travis and AppVeyor and require different parts of the software to work. This assures that we always have a stable version and improves code quality. \\
These tests are performed on remote servers and the status is visible on GitHub. \cite{githubci}

Travis and AppVeyor both use the same technology. They create a virtual machine to simulate a computer and run our software on that machine.



==> sections/opening_questions.tex <==
\begin{itemize}
	\item{Is it possible to combine NEAT and CNN?}
	\item{Is it possible to carefully explain the complexity of subjects and if possible, simplify them?}
	\item{Is it possible to cooperate and work with the hospital?}
	\item{Is it possible to evaluate mammographys at home with the software we possess?}
	\item{Is our software capable to emulate a human evolution?}
	\item{Is our software usable as an assistance system in the future?}
\end{itemize}


==> sections/our_targets.tex <==
 While working on our project we had to take our goals into account. So we found a lot oft them.  Here are our main goals.
\begin{itemize}
	\item{Read mammography correctly}
	\item{Probability indication to 95\%}
	\item{Visual display}
	\item{Present the knowledge to the layman}
	\item{Reach platform independency}
\end{itemize}
The ability to read mammography is very important because besides the project consisting of image recognition, it needs mammography too. Certainty is also really important for the project, and it puts a "stamp" on it because one has to be very sure before putting a cancer diagnose.\\
 A visual display is also a goal the project has, as it makes the use of the software easier and more appealing to the eye. A presentation for the layman could be a good supplement, providing them with the information they need, just to have a general clue. \\
 As a conclusion, our project should be softwate-independent with the purpose that one could be able to use it on any device.


==> sections/procedure.tex <==
\subsubsection{The beginning}

Our starting point was picking a topic for the project. \\
We haven't been dealing with this for quite a long time because we already had a concrete idea of what the project was going to be about. \\
Jan Hohenheim (project member) had an inspiring idea with which he truly inspired us. \\
Roughly one year before the project he had the idea to make possible the recognizing of different images using artificial intelligence.\\
In the course of this year, he collected information and experiences, and came up with a concept to make image recognition possible in the field of medicine, more precisely breast cancer (mammography). \\
When we started out the project, we had a very interesting topic and also someone who had previously dealt with it.\\

\subsubsection{The planning}

At the beginning, a rough plan of how the project is going to develop was made. \\
We have looked at the aspects which are very time-consuming and important. After this, we proceeded by making a weekly planning. \\
We knew what we had to do and how to do it, of course thanks to the planning but since that wouldn't be enough, we had to group each week and discuss tasks carefully.  \\
We also discussed how we would like to cooperate with the doctors.\\

\subsubsection{The realisation}

Since the planning has been completed, it was time for the realization. \\
As already mentioned in the planning, we worked in a weekly schedule. \\
This means that we divided all the big tasks into smaller ones, each one going on for about a week. \\
Having a really good overview of our project, we knew exactly where we stand. \\
Also we had a meeting every week and discussed our concerns about the project. \\
The biggest problem with the realization was that we lacked the computing power with which to run our project and visualize it. \\
We had a problem to present our project correctly and to make it clear to the people what we have achieved completing it. \\
Apart from this, the realization ran very well.\\
Our job was to mainly work on NEAT (NeuroEvolution of Augmenting Topologies) and CNN (Convolutional Neural Network). \\
When both parts were completed, it was our goal to connect them together. \\
In addition, we cooperated with a few doctors that helped us by providing us with data we needed.  \\
We searched for them on the internet and in books, at least the ones that were specialists in the field of oncology (tumor diseases). \\
We prepared a study protocol to present our project to the doctorsd. \\
After checking out our study protocol, Dr. Serafino Forte from the Hospital of Baden invited us to introduce him to our project. \\
He gave us some helpful tips and we discussed the next steps. \\

\subsubsection{The result}

The result led to a dichotomy. \\
The two largest parts, CNN (Convolutional Neural Network) and NEAT (NeuroEvolution of Augmenting Topologies), have been successfully connected together and they worked successfully. However, our computing power is much too low to test our software on. \\
One of our main concerns is to explain people who haven't encountered our program and this type of work that it would still run successfully, despite us not being able to show it to them or visualize it. \\
With the performance of a really good laptop, the learning of the network would still take about a half a year, which is  unfortunately time we don't have.\\

\subsubsection{Our conclusion}

Our software worked successfully and we are very satisfied with it. Unfortunately, we have used an outdated technology of mammography, which is nowadays almost to no longer needed. So it turns out that our software can serve in only a few facilities as an assistance system. However, this doesn't necessarily mean it's negative, quite the contrary - an advantage. Inserting the new technology is definitely possible, and therefore our software would also support all technologies.\\
In conclusion, our software can be used as an assistance system, but we want to optimize the data to make it easier for the doctors to work with it and eventually be able to help people thanks to the provided information. \\
The project was a very good opportunity to let our ideas run free and to further train our knowledge.  \\
We are very optimistic for our software to be used and in future optimized.\\


==> sections/progress.tex <==
\underline{Progress made until the end of October}\\
Implement the load of networks (ZAR)\\
Complete the visualizer (MFI)\\ 
Complete the documentation part ``How does a neural network work?'' (JST)

\underline{Progress made until the middle of November}\\
Complete the study journal (ZAR)\\
Complete CNN (JNF, JST)\\
Complete NEAT (ZAR, MFI)

\underline{Progress made until the end of November}\\
Complete the documentation part ``Automatic testing of software'' (JST)\\ Complete the documentation part ``What is NEAT?'' (MFI)

\underline{Progress made from the middle of November until the middle of December}\\
Connect CNN with NEAT (All)\\
Testing of different variations (All)\\
Execute benchmarks (All)\\
Possible tests in and cooperation with other people (All)

\underline{Progress made from mid to end of December}\\
Evaluation of tests, writing of conclusions (All)

\underline{Checkpoints}\\
16.11.2016: SGAICO Meeting- Deep Learning and Beyond\\
23.11.2016: Delivery of the fine concept (Table of contents)\\
18.01.2017: Delivery of the project and presentation\\
25.01.2017: Project exhibition\\


==> sections/targets.tex <==
While working on our project we had to make us mind about our targets. So we found a lot oft hem.  Here are our main targets.

1.	To read mammography\\
2.	Probability indication to 95\%\\
3.	Visual display\\
4.	Presentation for laity\\
5.	Platform independet\\


==> sections/what_is_neat.tex <==
NEAT stands for Evolving Neural Networks through Augmenting Topologies and is a technology first proposed by O. Stanley. \cite{Stanley2002} \\
It presents an elegant way to combine genetic algorithms with evolving topologies.


==> sections/working_programms_and_tools.tex <==
We have used the following platforms and programs for the work  Visual Studio; LaTex; and Github.\\

\subsubsection {Visual Studio}

Visual Studio is a programming tool developed by Microsoft for Windows we have programmed all of our software in. We have worked with it quite a lot as well. Since Visual Studio is very modern, it didn't cause us problems and without a doubt helped us with the project changes that we made.\\
Changes applied to the software structure were not too difficult.

\subsubsection {LaTex}

The tool we used for our documentation and design is LaTex, the advantages of which are that LaTex takes complete care of the presentation of the documentation, including the citations. This guarantees that we waste as little time as possible with visually designing the documentation. \\
Some rather special formulas can also be used wich the program formats it by itself so we don’t have to worry about it.\\

\subsubsection {Github}

Github is an online platform we used to store the code we have written in. In Github people can work on projects together and view other people's work. It can also work in a way that people give other people tasks or demand a review of a task. Github is and has been an enormous help to our project, beause it has given us an overview of the things we have programmed. On top of that, Github gives us reasssurement because every work has been checked and reviewed by some other member of the site. \\
In Github you can also make branches. A branch is a copy of a project. On one hand, it offers additional security for the programmer because if any changes are made in the original project, it can be possible that this would no longer works. On the other hand, if one is working on the branch, nothing can be destroyed. \\
Changes and edits in the branch can of course be made in the original project, but only if it's in order. Since our project was public on Github, people who had no idea about it, but were interested in it, could take a look at it. \\
Specialists in our area of expertise could look at our program and give us tips, for example on how to improve it. Github has many advantages and offers the user many possibilities.

